FP-Radar: Longitudinal Measurement and Early Detection of Browser Fingerprinting

Browser fingerprinting is a stateless tracking technique that attempts to combine information exposed by multiple different web APIs to create a unique identifier for tracking users across the web. Over the last decade, trackers have abused several existing and newly proposed web APIs to further enhance the browser fingerprint. Existing approaches are limited to detecting a specific fingerprinting technique(s) at a particular point in time. Thus, they are unable to systematically detect novel fingerprinting techniques that abuse different web APIs. In this paper, we propose FP-Radar, a machine learning approach that leverages longitudinal measurements of web API usage on top-100K websites over the last decade, for early detection of new and evolving browser fingerprinting techniques. The results show that FP-Radar is able to early detect the abuse of newly introduced properties of already known (e.g., WebGL, Sensor) and as well as previously unknown (e.g., Gamepad, Clipboard) APIs for browser fingerprinting. To the best of our knowledge, FP-Radar is also the first to detect the abuse of the Visibility API for ephemeral fingerprinting in the wild.

==> sections/table.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{@{}cclcccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{API}} & \multicolumn{1}{c}{\textbf{Keywords}} & \textbf{\begin{tabular}[c]{@{}c@{}}Browser \\ compatibility \\ Date\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Disclosure \\ Date\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Disclosure \\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Detection\\ Date*\end{tabular}} \\ \midrule
\multicolumn{2}{c}{\multirow{11}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Battery \\ Status\\  API\end{tabular}}}} & battery & \multirow{11}{*}{2014} & \multirow{11}{*}{2015} & \multirow{11}{*}{\begin{tabular}[c]{@{}c@{}}Paper \\ \textbackslash{}cite\{1\}\end{tabular}} & 2015 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & charging &  &  &  & 2015 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & chargingTime &  &  &  & 2015 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & chargingchange &  &  &  & 2017 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & chargingtimechange &  &  &  & 2017 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & dischargingTime &  &  &  & 2015 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & dischargingtimechange &  &  &  & 2017 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & getBattery &  &  &  & 2016 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & level &  &  &  & 2016 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & levelchange &  &  &  & 2016 \\ \cmidrule(lr){3-3} \cmidrule(l){7-7} 
\multicolumn{2}{c}{} & mozBattery &  &  &  & 2016 \\ \midrule
\multicolumn{2}{c}{\multirow{24}{*}{\textbf{Navigator}}} & appCodeName & 2003 & 2009 & \begin{tabular}[c]{@{}c@{}}Paper \\ \textbackslash{}cite\{2\}\end{tabular} & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & appName & 2003 & 2009 &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & appVersion & 2003 & 2009 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & buildID & 2018 & ?? &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & cookieEnabled & 2003 & 2009 &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & deviceMemory & 2017 & ?? &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & doNotTrack & 2011 & ?? &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & enabledPlugin &  & 2009 &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & hardwareConcurrency & 2014 & 2017 & \begin{tabular}[c]{@{}c@{}}Paper\\  \textbackslash{}cite\{4\}\end{tabular} & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & javaEnabled & 2003 & 2009 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & languages & 2014 & 2009 !!! &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & mimeTypes & 2003 & 2009 &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & oscpu & 2004 & 2009 &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & platform & 2003 & 2009 &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & plugins & 2003 & 2009 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & product & 2003 & ?? &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & productSub & 2003 & 2009 &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & standalone & ?? & ?? &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & suffixes & 2004 & 2009 &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & taintEnabled & 2004 & 2009 &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & userAgent & 2003 & 2009 &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & vendor & 2003 & 2009 &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & vendorSub & 2004 & ?? &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & webdriver & 2015 & ?? &  & 2017 \\ \midrule
\multicolumn{2}{c}{\multirow{10}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Geolocation\\  API\end{tabular}}}} & altitude & 2009 & 2008 & \begin{tabular}[c]{@{}c@{}}W3C \\ Documentation \\ \textbackslash{}cite\{?\}\end{tabular} & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & altitudeAccuracy & 2009 & 2008 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & clearWatch & 2009 & 2008 &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & geolocation & 2009 & 2008 &  & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & latitude & 2009 & 2008 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & longitude & 2009 & 2008 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & PERMISSION\_DENIED & 2009 & 2008 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & POSITION\_UNAVAILABLE & 2009 & 2008 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & speed & 2009 & 2008 &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & watchPosition & 2009 & 2008 &  & 2019 \\ \midrule
\multicolumn{1}{l}{\multirow{25}{*}{\textbf{Storage}}} & \multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Web \\ Storage \\ API\end{tabular}}} & localStorage & 2009 & 2010 & Paper \textbackslash{}cite\{3\} & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & window.sessionStorage & 2006 & 2010 & Paper \textbackslash{}cite\{3\} & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & setItem & 2009 & ?? &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & storageArea & 2006 & ?? &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & Storage & 2009 & ?? &  & 2015 \\ \cmidrule(l){2-7} 
\multicolumn{1}{l}{} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Storage\\  API\end{tabular}}} & persist & 2016 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & navigator.storage & 2016 & ?? &  & 2015 \\ \cmidrule(l){2-7} 
\multicolumn{1}{l}{} & \multirow{18}{*}{\begin{tabular}[c]{@{}c@{}}IndexedDB\\  API\end{tabular}} & bound & 2012 & ?? &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & cmp & 2012 & ?? &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & createObjectStore & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & deleteDatabase & 2012 & ?? &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & IDBDatabase & 2012 & ?? &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & IDBKeyRange & 2012 & ?? &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & IDBRequest & 2012 & ?? &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & IDBTransaction & 2012 & ?? &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & \begin{tabular}[c]{@{}l@{}}WindowOrWorker\\ GlobalScope.\\ IndexedDB\end{tabular} & 2012 & ?? &  & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & keyPath & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & lower & 2012 & ?? &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & objectStore & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & objectStoreNames & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & onsuccess & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & onupgradeneeded & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & setVersion & 2012 & ?? &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & storeName & 2012 & ?? &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{1}{l}{} &  & transaction & 2012 & ?? &  & 2015 \\ \midrule
\multicolumn{2}{c}{\multirow{61}{*}{\textbf{WebGL (1,2) API}}} & ANGLE\_instanced\_arrays & 2014 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & attachShader & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & bindBuffer & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & bufferData & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & clearColor & 2011 &  &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & compileShader & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & createProgram & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & createQuery & 2017 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & createShader & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & depthFunc & 2011 &  &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & drawArrays & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & enable & 2011 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & enableVertexAttribArray & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & EXT\_blend\_minmax & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & EXT\_color\_buffer\_half\_float & 2016 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & EXT\_disjoint\_timer\_query & 2015-2018 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & EXT\_frag\_depth & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & EXT\_sRGB & 2013 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}EXT\_texture\_filter\\ \_anisotropic\end{tabular} & 2013 &  &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}FRAGMENT\_SHADER\_\\ DERIVATIVE\_HINT\_OES\end{tabular} & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getAttribLocation & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getContextAttributes & 2011 &  &  & 2015 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getError & 2011 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getExtension & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getProgramParameter & 2011 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getShaderPrecisionFormat & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getSupportedExtensions & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getUniformLocation & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & isBuffer & 2011 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & lineWidth & NO -IE-2013 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & linkProgram & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}MAX\_COLOR\_\\ ATTACHMENTS\_WEBGL\end{tabular} & 2014 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}MAX\_DRAW\_BUFFERS\\ \_WEBGL\end{tabular} & 2014 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}MAX\_TEXTURE\_MAX\\ \_ANISOTROPY\_EXT\end{tabular} & 2014 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & OES\_element\_index\_uint & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & OES\_standard\_derivatives & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & OES\_texture\_float & 2011 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & OES\_texture\_float\_linear & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & OES\_texture\_half\_float & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & OES\_vertex\_array\_object & 2013 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & precision & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & rangeMax & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & rangeMin & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & shaderSource & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & statusMessage & 2011 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & useProgram & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & vertexAttribPointer & 2011 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & viewport & 2011 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & webgl & 2011 & 2012 & Paper \textbackslash{}cite\{5\} & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WEBGL\_color\_buffer\_float & 2014 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}WEBGL\_compressed\\ \_texture\_astc\end{tabular} & 2014 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}WEBGL\_compressed\\ \_texture\_etc1\end{tabular} & 2014 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}WEBGL\_compressed\\ \_texture\_s3tc\end{tabular} & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & \begin{tabular}[c]{@{}l@{}}WEBGL\_debug\_\\ renderer\_info\end{tabular} & 2014 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WEBGL\_debug\_shaders & 2014 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WEBGL\_depth\_texture & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WEBGL\_draw\_buffers & 2014 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WEBGL\_lose\_context & 2013 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WebGL2RenderingContext & 2017 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WebGLContextEvent & 2011 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & WebGLRenderingContext & 2011 &  &  & 2011 \\ \midrule
\multicolumn{2}{c}{\multirow{41}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Resource \\ Timing\\ API\end{tabular}}}} & clearMarks & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & clearMeasures & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & connectEnd & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & connectStart & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & decodedBodySize & 2016 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domComplete & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domContentLoadedEventEnd & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domContentLoadedEventStart & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domInteractive & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domLoading & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domainLookupEnd & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & domainLookupStart & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & encodedBodySize & 2016 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & entryType & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & fetchStart & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getEntries & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getEntriesByName & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getEntriesByType & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & initiatorType & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & loadEventEnd & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & loadEventStart & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & mark & 2013 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & measure & 2013 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & navigationStart & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & now & 2012 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & nextHopProtocol & 2016 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & paint & 2017 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & Performance & 2010 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & redirectCount & 2011 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & redirectEnd & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & redirectStart & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & requestStart & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & responseEnd & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & responseStart & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & secureConnectionStart & 2015 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & serverTiming & 2018 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & timing & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & transferSize & 2016 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & unloadEventEnd & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & unloadEventStart & 2010 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & workerStart & 2015 &  &  & 2019 \\ \midrule
\multicolumn{2}{c}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Page Visibility\\ API\end{tabular}}}} & focused & 2013 & 2020 & \begin{tabular}[c]{@{}c@{}}Whit Paper\\ \textbackslash{}cite\{10\}\end{tabular} & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & prerender & 2013 & 2020 &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & visibilityState & 2013 & 2020 &  & 2017 \\ \midrule
\multicolumn{2}{l}{\multirow{6}{*}{\textbf{Web Worker API}}} & applicationCache & 2010 &  &  & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & btoa & 2007 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & importScripts & 2009 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & isSecureContext & 2016 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & Worker & 2009 &  &  & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & Worklet & 2018 &  &  & 2018 \\ \midrule
\multicolumn{2}{l}{\multirow{8}{*}{\textbf{XMLHttpRequest}}} & getAllResponseHeaders & 2004 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & overrideMimeType & 2004 &  &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & responseText & 2004 &  &  & 2011 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & responseType & 2011 &  &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & responseURL & 2014 &  &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & responseXML & 2004 &  &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & statusText & 2004 &  &  & 2013 \\ \cmidrule(l){3-7} 
\multicolumn{2}{l}{} & XMLHttpRequest & 2004 &  &  & 2013 \\ \midrule
\multicolumn{2}{c}{\multirow{3}{*}{\textbf{GamePad API}}} & Gamepad & 2014 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & getGamepads & 2014 & 2020 & \begin{tabular}[c]{@{}c@{}}https://hacks.mozilla.org\\ /2020/07/securing-gamepad-api/\end{tabular} & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & mapping & 2014 &  &  & 2017 \\ \midrule
\multicolumn{2}{c}{\multirow{14}{*}{\textbf{Mouse}}} & dblclick & 2007 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & deltaX & 2012 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & deltaY & 2012 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & deltaZ & 2012 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & DOMMouseScroll & 2004(only Firefox) &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & initMouseEvent & 2005 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & mousewheel & 2007 &  &  & 2019 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & movementX & 2014 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & movementY & 2014 &  &  & 2016 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & onmousemove & 2003 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & requestPointerLock & 2014 &  &  & 2014 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & scrollX & 2003 &  &  & 2017 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & scrollY & 2003 &  &  & 2018 \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & wheelDelta & 2008 &  &  & 2018 \\ \midrule
\multicolumn{2}{c}{\multirow{4}{*}{\textbf{TouchEvent}}} & force & \multicolumn{1}{l}{2012} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2013} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & ontouchstart & \multicolumn{1}{l}{2011 (Safari iOS)} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2011} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & rotationAngle & \multicolumn{1}{l}{2015} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2017} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & TouchEvent & \multicolumn{1}{l}{2012} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2015} \\ \midrule
\multicolumn{2}{c}{\multirow{7}{*}{\textbf{Sensor API}}} & AbsoluteOrientationSenso & \multicolumn{1}{l}{2018} & \multicolumn{1}{l}{2014} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2018} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & acceleration & \multicolumn{1}{l}{2011} & \multicolumn{1}{l}{2014} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2017} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & accelerationIncludingGravity & \multicolumn{1}{l}{2011} & \multicolumn{1}{l}{2014} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2018} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & devicemotion & \multicolumn{1}{l}{2011} & \multicolumn{1}{l}{2014} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2017} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & DeviceMotionEvent & \multicolumn{1}{l}{2014} & \multicolumn{1}{l}{2014} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2018} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & DeviceOrientationEvent & \multicolumn{1}{l}{2010} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2017} \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{} & rotationRate & \multicolumn{1}{l}{2011} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2018} \\ \midrule
\multicolumn{2}{c}{\multirow{3}{*}{\textbf{Clipboard API}}} & copy & \multicolumn{1}{l}{2007} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2019} \\
\multicolumn{2}{c}{} & clipboardData & \multicolumn{1}{l}{2013} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2018} \\
\multicolumn{2}{c}{} & paste & \multicolumn{1}{l}{2007} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{2019}
\end{tabular}
\end{table*}


\begin{coment}
\begin{table*}[!h]
\centering
\begin{tabular}{c|c|c|c|c|l}
\multirow{2}{*}{\textbf{Cluster label}} & \textbf{Life-span} & \textbf{\% keywords in} & \textbf{\# keywords in} & \textbf{\# keywords in} & \multirow{2}{*}{\textbf{Dominant APIs}}\\
 & \textbf{in years} & \textbf{in FP scripts} & \textbf{fingerprintjs2} & \textbf{only FP scripts} & \\\hline
Fingerprinting & 9 & \textbf{63\%} & \textbf{99} & \textbf{48} & Battery, Navigator, Network Information \\\hline
Other & 5 & 23\% & 4 & 4 & FullScreen, VideoTrack, HTMLMediaElement\\\hline
Other & 4 & 20\% & 5 & 3 & Long Tasks, Resource Timing, Background Tasks \\\hline
Other & 4 & 11\% & 5 & 0 & VideoTrack, Geolocation, Long Tasks \\\hline
Other & 4 & 2\% & 2 & 0 & History, HTMLElement, HTMLTableElement \\\hline
Other & 10 & 20\% & 8 & 1 & HTMLIFrameElement, Navigator, URL \\\hline
Other & 5 & 15\% & 7 & 0 & Visual Viewport, Web Crypto, Channel Messaging \\\hline
Other & 9 & 18\% & 7 & 1 & Resource Timing, Page Visibility, History \\\hline
Other & 6 & 17\% & 9 & 9 & Mouse, TouchEvents, Canvas \\\hline
Other & 4 & 3\% & 3 & 0 & Sensors, Gamepad, Fullscreen, Web Bluetooth \\\hline
Other & 4 & 15\% & 3 & 3 & XMLSerializer, Mouse, ShadowRoot \\\hline
Other & 4 & 3\% & 2 & 4 & FileReader, Web Animations, XMLHttpRequest \\\hline
Other & 4 & 10\% & 3 & 0 & Fetch API, Notification, NodeFilter \\\hline
Other & 4 & 11\% & 5 & 5 & CSS Painting, XMLHTTPRequest \\\hline
Other & 4 & 3\% & 2 & 4 & Long Tasks, Resource Timing, Background Tasks \\\hline

\end{tabular}
\caption{Temporal clusters detected by \name and their key characteristics. The fingerprinting cluster clearly stands out as compared to the remaining clusters in terms of its similarity with known fingerprinting scripts.}

\vspace{-.1in}
\end{table*}
\end{coment}



==> sections/tmp_clustering_results.tex <==
Using the temporal clustering algorithm described in Section \ref{ZeroDay}, we extract 78 temporal clusters in total.
%
To reduce the overhead of manually analyzing temporal clusters, we filter out short-lived temporal clusters whose time duration is less than three years.
%To reduce the overhead of manually analyzing temporal clusters, we filter out unviable clusters based on the following criterion.
%
%First, we filter out short-lived temporal clusters whose time duration is less than three years.
%
Figure \ref{pruning} shows that 18\% of temporal clusters have time duration more than two years.
%
%Second, amongst the long-lived clusters, we filter out the small temporal clusters, whose corresponding static clusters contain fewer than 10 API keywords.
%
%Figure \ref{pruning:size} shows that 3\% of long-lived temporal clusters have less than 10 API keyword.
%
After the filtering, we are left with 14 viable temporal clusters that are visualized in Figure \ref{temporal_clusters}(b).
%
Each temporal cluster is shown by an alphabetic character.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/duration.pdf}
  \caption{Life cycle of Temporal Clusters}
  \label{pruning}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\textbf{P2:} Explain how we detect FP communities.
Next, we label the temporal clusters with fingerprinting or non-fingerprinting category using the criteria described in Section \ref{ZeroDay}. 
%
To this end, we use static clusters in 2019 because we have access to valid ground truth from \cite{iqbal2020fingerprinting}.
%
Out of 5 viable static clusters in 2019, one of them satisfies the three criteria: 
%
(1) 67\% of its API keywords are common with the fingerprintjs2 library, 
%
(2) 45\% of its API keywords have the frequency ratio of appearance in fingerprinting to non-fingerprinting scripts more than 16, 
%
and (3) 28 of its API keywords is only observed in fingerprinting scripts. 
%
The static clusters in previous years that are connected to the static fingerprinting cluster in 2019 (based on the similarity algorithm in Section \ref{Temporal_Clustering_algo}) are also labeled as fingerprinting. 
%
Considering temporal clusters \textit{G} and \textit{H} in Figure \ref{temporal_clusters}(b), we can observe that that two clusters in 2018 are merged to one cluster in 2019. 
%
This results in labeling two temporal clusters out of the 15 viable clusters as fingerprinting.
%
One starting from 2011 to 2019 and the other merges from 2018 with the 2019.
%
Moreover, the temporal cluster \textit{G} does not have a consecutive static cluster in 2012.
%
This could have two reasons. 
%
First since our data is collected using Wayback machine, sometimes it fails to properly archive all web pages, particularly for initial years.
%
As a result, we might lose some data here.
%
Second, although the first studies proved that browser fingerprinting is possible goes back to 2009 \cite{mayer2009any}, the prevalence of abusing APIs for fingerprinting just goes back to recent years \cite{lerner2016internet} 
%
Consequently, fewer APIs are available in the early years that had been abused for fingerprinting techniques.
%

On the other hand, the static clusters in previous years connected to the fingerprinting cluster in 2019 also satisfy the above mentioned criteria better than other static clusters in non fingerprinting temporal clusters.
%
%Specifically, by average  .... for fingerprinting cluster is more than the average for non-fingerprinting %clusters?
%
Specifically, 66\% (vs. 3\%) of the API keywords are on average common with the fingerprintjs2 library, 172 (vs. 4) of API keywords in each step community has a frequency ratio of appearance in fingerprinting to non-fingerprinting scripts more than 16, and by average 47 (vs. 2) of the API keywords are only observed in fingerprinting scripts in the fingerprinting static clusters (as compared to non-fingerprinting static clusters). 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/temporal_cluster_labels.pdf}
  \caption{Evolution of temporal Clusters contain API keywords along side top-5 dominant APIs inside them}
  \label{temporal_clusters}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Yet, the compatibility of two approaches, i.e. Similarity algorithm and three criteria as we mentioned in Section \ref{ZeroDay}, in detecting the temporal fingerprinting cluster is not far beyond our expectation.
%
The reason behind this is that although fingerprinting techniques are changing over the time, this change is not sudden.
%
Fingerprinting cluster gradually change over the time.
%
In the following we will show that our technique is able to monitor the evolution of fingerprinting cluster over the time with high accuracy.
%
%Thus, we conclude that although we do not have ground truth for previous years and we just rely on the similarity to detect the fingerprinting temporal cluster, 


\textbf{Labeling temporal clusters: }\label{section:labeling} Having the temporal clusters, we now analyse the API keywords inside each temporal cluster to figure out is there any reason behind clustering?
%
In another words, we are more interested in detecting whether we can assign a particular function to each temporal cluster.
%
To this end, we crawl MDN Web docs \cite{MDN_API} to create a hierarchical glossary of APIs, Interfaces and corresponding Keywords.
%
Specifically, we first crawl all 1028 interfaces on MDN Web docs and collect all the corresponding keywords for each interface including properties, values, constant names, attributes, method names, event names, and error names.
%
Then we crawl all 88 APIs to figure out what interfaces are engaged in implementing an API. 
%
This comprehensive glossary enables us to map each API keyword inside each dynamic cluster to its corresponding interface and API. 
%
%
In Listing \ref{interface-example} we provide a partial view of related interfaces and keywords for \texttt{Push} API.
%
For the sake of integrity, we remove keywords or interfaces which appear in multiple interfaces or APIs correspondingly.
%
As an example, we remove a keyword like \textit{length} which belongs to 54 different interfaces. 
%
Otherwise, we are not able to map each API keyword to a unique interface or API.
%
At the next step, to find dominant APIs inside each temporal cluster, we calculate the frequency of each API callings and normalize them by dividing their frequency to the total number of static communities in each temporal cluster multiply by total number of keywords and interfaces of the corresponding API. 
%
As an example, consider \texttt{WebGL} API in temporal fingerprinting cluster with 8 step communities.
%
This API consists of 48 interfaces and 301 keywords in total.
%
Since 2010 to 2019, it has been called 211 times.
%
Therefore the normal and average frequency of this interface during the fingerprinting cluster is $211 / ((48+301+1) \times 8) * 100 = 7\%$.
%
This indicates that $7\%$ of the API keywords in temporal fingerprinting cluster calls \texttt{WebGL} API.
\begin{listing}
\begin{lstlisting}
"Push_API": 
{   
    "interfaces": [
        "PushSubscriptionOptions",
        "PushSubscription",
        "PushManager"]
    "keywords" : [
            "registrations",
            "subscriptionId",
            "getSubscription",
            "endpoint",
            "hasPermission", ...]
}
\end{lstlisting}
\caption{Push API} 
\label{interface-example}
\end{listing}
% 36.Stating that your results confirm previous evidence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

